Making Theft Useless: Adulteration-Based Protection of Proprietary Knowledge Graphs in GraphRAG Systems

Graph Retrieval-Augmented Generation (GraphRAG) has emerged as a key technique for enhancing Large Language Models (LLMs) with proprietary Knowledge Graphs (KGs) in knowledge-intensive applications. As these KGs often represent an organization's highly valuable intellectual property (IP), they face a significant risk of theft for private use. In this scenario, attackers operate in isolated environments. This private-use threat renders passive defenses like watermarking ineffective, as they require output access for detection. Simultaneously, the low-latency demands of GraphRAG make strong encryption which incurs prohibitive overhead impractical. To address these challenges, we propose AURA, a novel framework based on Data Adulteration designed to make any stolen KG unusable to an adversary. Our framework pre-emptively injects plausible but false adulterants into the KG. For an attacker, these adulterants deteriorate the retrieved context and lead to factually incorrect responses. Conversely, for authorized users, a secret key enables the efficient filtering of all adulterants via encrypted metadata tags before they are passed to the LLM, ensuring query results remain completely accurate. Our evaluation demonstrates the effectiveness of this approach: AURA degrades the performance of unauthorized systems to an accuracy of just 5.3%, while maintaining 100% fidelity for authorized users with negligible overhead. Furthermore, AURA proves robust against various sanitization attempts, retaining 80.2% of its adulterants.

==> items/table_predict_model.tex <==
\begin{table}[h]
    \centering
    \caption{Impact of Link Prediction Models}
    \renewcommand{\arraystretch}{1.2}
    \setlength{\tabcolsep}{8pt}
    \begin{tabular}{lccc}
        \toprule
        \textbf{Model} & \textbf{MetaQA} & \textbf{WebQSP} & \textbf{HotpotQA} \\
        \midrule
        TransE & 98.0\% & 98.6\% & 98.8\% \\
        RotatE & 98.2\% & 98.5\% & 99.1\% \\
        ConvE  & 98.4\% & 98.4\% & 99.1\% \\
        \bottomrule
    \end{tabular}
    \label{tab:predict_model_impact}
\end{table}

==> items/table_retriever.tex <==
\begin{table}[h]
    \centering
    \caption{Impact of Retriever}
    \renewcommand{\arraystretch}{1.2}
    \setlength{\tabcolsep}{8pt}
    \resizebox{1.0\linewidth}{!}{
        \begin{tabular}{lccc}
            \toprule
            \textbf{Retriever} & \textbf{MetaQA} & \textbf{WebQSP} & \textbf{HotpotQA} \\
            \midrule
            NER-based Symbolic & 98.5\% & 98.4\% & 99.0\% \\
            Dense Vector & 98.2\% & 98.5\% & 99.1\% \\
            Hybrid & 98.3\% & 98.3\% & 98.6\% \\
            \bottomrule
        \end{tabular}}
    \label{tab:retriever_impact}
\end{table}

==> items/table_robustness_KGE.tex <==
\begin{table}[t]
    \centering
    \caption{KGE-based Sanitization Attack}
    \renewcommand{\arraystretch}{1.2}
    \setlength{\tabcolsep}{3pt}
    \resizebox{1.0\linewidth}{!}{ % Adjusted width for a better fit
    \begin{tabular}{lcc}
        \toprule
        \textbf{Detection Method} & \textbf{Detected Samples} & \textbf{Retain Percentage} \\
        \midrule
        KGE-based Sanitization Attack & 49,925 & 80.2\% \\
        \bottomrule
    \end{tabular}}
    \label{tab:robustness_kge}
\end{table}

==> items/table_robustness_hybrid.tex <==
\begin{table}[t]
    \centering
    \caption{Hybrid Feature-based Attack}
    \renewcommand{\arraystretch}{1.2}
    \setlength{\tabcolsep}{3pt}
    \resizebox{1.0\linewidth}{!}{ % Adjusted width for a better fit
    \begin{tabular}{lcc}
        \toprule
        \textbf{Detection Method} & \textbf{Detected Samples} & \textbf{Retain Percentage} \\
        \midrule
        Hybrid Feature-based Attack& 13,758 & 94.5\% \\
        \bottomrule
    \end{tabular}}
    \label{tab:robustness_hybrid}
\end{table}
